EZ-SP: Fast and Lightweight Superpoint-Based 3D Segmentation

Superpoint-based pipelines provide an efficient alternative to point- or voxel-based 3D semantic segmentation, but are often bottlenecked by their CPU-bound partition step. We propose a learnable, fully GPU partitioning algorithm that generates geometrically and semantically coherent superpoints 13$\times$ faster than prior methods. Our module is compact (under 60k parameters), trains in under 20 minutes with a differentiable surrogate loss, and requires no handcrafted features. Combine with a lightweight superpoint classifier, the full pipeline fits in $<$2 MB of VRAM, scales to multi-million-point scenes, and supports real-time inference. With 72$\times$ faster inference and 120$\times$ fewer parameters, EZ-SP matches the accuracy of point-based SOTA models across three domains: indoor scans (S3DIS), autonomous driving (KITTI-360), and aerial LiDAR (DALES). Code and pretrained models are accessible at github.com/drprojects/superpoint_transformer.

==> figures/graph.tex <==
\node [thick, draw=black, circle, heat fill=\valA, minimum size=5mm] (n1) at (0,1) {};
\node [thick, draw=black, circle, heat fill=\valB, minimum size=5mm] (n2) at (1,2) {};
\node [thick, draw=black, circle, heat fill=\valC, minimum size=5mm] (n3) at (1,0) {};
\node [thick, draw=black, circle, heat fill=\valD, minimum size=5mm] (n4) at (2,1) {};
\node [thick, draw=black, circle, heat fill=\valE, minimum size=5mm] (n5) at (3,0) {};
\node [thick, draw=black, circle, heat fill=\valF, minimum size=5mm] (n6) at (4,1) {};
\node [thick, draw=black, circle, heat fill=\valG, minimum size=5mm] (n7) at (3,2) {};

==> figures/quali_seg_bk.tex <==

\begin{tabular}{l@{}c@{}c@{}c}

\raiseandrotate{1.8}{Input} 
&
\includegraphics[width=0.29\linewidth, height=0.2\linewidth]{images/prediction/s3dis_pcp_Area_5__center=2_15_0__radius=5_rgb_colors.jpg}
&
\includegraphics[width=0.29\linewidth, height=0.2\linewidth]{images/prediction/kitti360_ezsp_0000000372_0000000610__center=-150_34_-2__radius=15_rgb_colors.jpg}
&
\includegraphics[width=0.29\linewidth, height=0.2\linewidth]{images/prediction/dales_ezsp_5175_54395_new__TILE_3-3_OF_3-3__center=7_350_-3__radius=32_intensity_colors.jpg}
\\
\raiseandrotate{0.4}{Ground Truth} 
&
\includegraphics[width=0.29\linewidth, height=0.2\linewidth]{images/prediction/s3dis_pcp_Area_5__center=2_15_0__radius=5_y_colors.jpg}
&
\includegraphics[width=0.29\linewidth, height=0.2\linewidth]{images/prediction/kitti360_ezsp_0000000372_0000000610__center=-150_34_-2__radius=15_y_colors.jpg}
&
\includegraphics[width=0.29\linewidth, height=0.2\linewidth]{images/prediction/dales_ezsp_5175_54395_new__TILE_3-3_OF_3-3__center=7_350_-3__radius=32_y_colors.jpg}
\\
\raiseandrotate{0.6}{Prediction} 
&
\includegraphics[width=0.29\linewidth, height=0.2\linewidth]{images/prediction/s3dis_ezsp_Area5__center=2_15_0__radius=5_pred_colors.jpg}
&
\includegraphics[width=0.29\linewidth, height=0.2\linewidth]{images/prediction/kitti360_ezsp_0000000372_0000000610__center=-150_34_-2__radius=15_pred_colors.jpg}
&
\includegraphics[width=0.29\linewidth, height=0.2\linewidth]{images/prediction/dales_ezsp_5175_54395_new__TILE_3-3_OF_3-3__center=7_350_-3__radius=32_pred_colors.jpg}
\\
&
\begin{tabular}{@{\hspace{-4mm}}r@{\,}l@{\;}r@{\,}l@{\;}r@{\,}l@{\;}r@{\,}l@{\;}r@{\,}l@{\;}@{}}
            \definecolor{tempcolor}{rgb}{.37,0.61,0.77}
            \tikz[baseline=+0.3 ex] \fill[fill=tempcolor, scale=0.25,  draw=black] (0, 0) rectangle (1.2, 1.2); 
            & \scriptsize{floor}
            &
            \definecolor{tempcolor}{rgb}{0.70,0.45,0.31}
            \tikz[baseline=+0.3 ex] \fill[fill=tempcolor, scale=0.25,  draw=black] (0, 0) rectangle (1.2, 1.2); 
            & \scriptsize{wall}
            &
            \definecolor{tempcolor}{rgb}{0.31,0.63,.58}
            \tikz[baseline=+0.3 ex] \fill[fill=tempcolor, scale=0.25,  draw=black] (0, 0) rectangle (1.2, 1.2);
            & \scriptsize{column} 
            &
            \definecolor{tempcolor}{rgb}{0.30,0.68,.32}
            \tikz[baseline=+0.3 ex] \fill[fill=tempcolor, scale=0.25,  draw=black] (0, 0) rectangle (1.2, 1.2); 
            & \scriptsize{wind.}
            &
            \definecolor{tempcolor}{rgb}{.42,0.52,0.29}
            \tikz[baseline=+0.3 ex] \fill[fill=tempcolor, scale=0.25,  draw=black] (0, 0) rectangle (1.2, 1.2); 
            & \scriptsize{door}
            \\
            \definecolor{tempcolor}{rgb}{.16,0.19,0.39}
            \tikz[baseline=+0.3 ex] \fill[fill=tempcolor, scale=0.25,  draw=black] (0, 0) rectangle (1.2, 1.2);
            & \scriptsize{chair}
            &
            \definecolor{tempcolor}{rgb}{.30,0.30,0.30}
            \tikz[baseline=+0.3 ex] \fill[fill=tempcolor, scale=0.25,  draw=black] (0, 0) rectangle (1.2, 1.2);
            & \scriptsize{table} 
            &
            \definecolor{tempcolor}{rgb}{.88,0.20,0.20}
            \tikz[baseline=+0.3 ex] \fill[fill=tempcolor, scale=0.25,  draw=black] (0, 0) rectangle (1.2, 1.2); 
            & \scriptsize{bookcase}
            &
            \definecolor{tempcolor}{rgb}{.32,0.43,.45}
            \tikz[baseline=+0.3 ex] \fill[fill=tempcolor, scale=0.25,  draw=black] (0, 0) rectangle (1.2, 1.2);
            & \scriptsize{board}
            &
            \definecolor{tempcolor}{rgb}{0.91,0.91,.90}
            \tikz[baseline=+0.3 ex] \fill[fill=tempcolor, scale=0.25,  draw=black] (0, 0) rectangle (1.2, 1.2);
            & \scriptsize{clut.} 
        \end{tabular}
&
\begin{tabular}{@{}r@{\,}l@{\;}r@{\,}l@{\;}r@{\,}l@{\;}r@{\,}l@{\;}@{}}
            \definecolor{tempcolor}{rgb}{0.50, 0.25, 0.50}
            \tikz[baseline=+0.3 ex] \fill[fill=tempcolor, scale=0.25,  draw=black] (0, 0) rectangle (1.2, 1.2);
            & \scriptsize{road} 
            &
            \definecolor{tempcolor}{rgb}{0.95, 0.13, 0.90}
            \tikz[baseline=+0.3 ex] \fill[fill=tempcolor, scale=0.25,  draw=black] (0, 0) rectangle (1.2, 1.2);
            & \scriptsize{sidewalk} 
            &
            \definecolor{tempcolor}{rgb}{0.27, 0.27, 0.27}
            \tikz[baseline=+0.3 ex] \fill[fill=tempcolor, scale=0.25,  draw=black] (0, 0) rectangle (1.2, 1.2);
            & \scriptsize{building} 
            &
            \definecolor{tempcolor}{rgb}{0.4 , 0.4 , 0.61}
            \tikz[baseline=+0.3 ex] \fill[fill=tempcolor, scale=0.25,  draw=black] (0, 0) rectangle (1.2, 1.2);
            & \scriptsize{wall} 
            \\
            \definecolor{tempcolor}{rgb}{0.74, 0.6 , 0.6 }
            \tikz[baseline=+0.3 ex] \fill[fill=tempcolor, scale=0.25,  draw=black] (0, 0) rectangle (1.2, 1.2);
            & \scriptsize{fence} 
            &
            \definecolor{tempcolor}{rgb}{0.41, 0.55, 0.13}
            \tikz[baseline=+0.3 ex] \fill[fill=tempcolor, scale=0.25,  draw=black] (0, 0) rectangle (1.2, 1.2);
            & \scriptsize{vegetation} 
            &
            \definecolor{tempcolor}{rgb}{0.59, 0.98, 0.59}
            \tikz[baseline=+0.3 ex] \fill[fill=tempcolor, scale=0.25,  draw=black] (0, 0) rectangle (1.2, 1.2);
            & \scriptsize{terrain} 
            &
            \definecolor{tempcolor}{rgb}{0.  , 0.  , 0.55}
            \tikz[baseline=+0.3 ex] \fill[fill=tempcolor, scale=0.25,  draw=black] (0, 0) rectangle (1.2, 1.2);
            & \scriptsize{car} 
        \end{tabular}
&
\begin{tabular}{r@{\,}l@{\;}r@{\,}l@{\;}r@{\,}l@{\;}}
            \definecolor{tempcolor}{rgb}{0.95, 0.84, 0.67}
            \tikz[baseline=+0.3 ex] \fill[fill=tempcolor, scale=0.25,  draw=black] (0, 0) rectangle (1.2, 1.2);
            & \scriptsize{ground} 
            &
            \definecolor{tempcolor}{rgb}{0.27, 0.45, 0.26}
            \tikz[baseline=+0.3 ex] \fill[fill=tempcolor, scale=0.25,  draw=black] (0, 0) rectangle (1.2, 1.2); 
            & \scriptsize{vegetation}
            &
            \definecolor{tempcolor}{rgb}{0.91, 0.20, 0.94}
            \tikz[baseline=+0.3 ex] \fill[fill=tempcolor, scale=0.25,  draw=black] (0, 0) rectangle (1.2, 1.2); 
            & \scriptsize{car}
            \\
            \definecolor{tempcolor}{rgb}{0., 0.91,  0.04}
            \tikz[baseline=+0.3 ex] \fill[fill=tempcolor, scale=0.25,  draw=black] (0, 0) rectangle (1.2, 1.2); 
            & \scriptsize{fence}
            &
            \definecolor{tempcolor}{rgb}{0.84, 0.26, 0.21}
            \tikz[baseline=+0.3 ex] \fill[fill=tempcolor, scale=0.25,  draw=black] (0, 0) rectangle (1.2, 1.2);
            & \scriptsize{building}
            & 
            \definecolor{tempcolor}{rgb}{0, 0, 0}
            \tikz[baseline=+0.3 ex] \fill[fill=tempcolor, scale=0.25,  draw=black] (0, 0) rectangle (1.2, 1.2);
            & \scriptsize{unlabelled}  
        \end{tabular}
\\
&
\begin{subfigure}{.25\linewidth}
    \label{fig:quali:s3dis}
    \caption{S3DIS}
\end{subfigure}
&
\begin{subfigure}{.25\linewidth}
    \label{fig:quali:kitti}
    \caption{KITTI360}
\end{subfigure}
&
\begin{subfigure}{.25\linewidth}
    \label{fig:quali:dales}
    \caption{DALES}
\end{subfigure}
\end{tabular}




==> sections/3_method.tex <==
\subsection{x}

\begin{figure*}
    \centering
    \resizebox{\linewidth}{!}{
    \input{figures/pipeline}
    }
    %\input{figures/table}
   \caption{\textbf{Proposed pipeline.} 
A lightweight 3D backbone embeds every point of the input scan into a low-dimensional feature space.  
A differentiable clustering stage predicts \emph{transition edges}—edges that likely cross semantic boundaries—and groups points into semantically homogeneous superpoints.  
A superpoint-level segmentation head then assigns a class label to each superpoint, which is finally propagated back to the original points to yield dense semantic predictions.}
    \label{fig:enter-label}
\end{figure*}

$\cP$ point clouds, dim $P \times 3+F$
$F=0, 1$ or $3$

\para{Point Embedding.} Embedding function 
$\phi^{\text{point}}:\cP \mapsto P \times M $ associate each point with an embedding of size $M$
lightweight local pointwise encoder, typically a few sparse convs

\para{Partitioning.} We use the mean-shift algorithm to spatially smooth the point features $\cF^{(0)}=\phi^{\text{point}}(\cP)$ for $I$ iteration $i=1\cdots I$:
\begin{align}
    \cF^{(i+1)}_p 
    &= 
    \frac
    {
    \sum_{q \in \mathcal{N}(p)}
    \omega_{p,q}^{(i)}
    \cF^{(i)}_q
    }
    {
    \sum_{q \in \mathcal{N}(p)}\omega_{p,q}^{(i)}
    }
    ~,
\end{align}
where 
$ \omega_{p,q}^{(i)}= \exp
    \left(-\Vert
        \cF^{(i)}_p
        -
        \cF^{(i)}_q
\Vert^2/ \sigma^2\right)$ and $\sigma>0$ an hyperparameter.
After $I$ iterations, we define the semantic divergence $d(p,q) \in [0,1]$ between two adjacent points as:
\begin{align}
    d(p,q) = 
    \frac
    {
    \Vert
        \cF^{(I)}_p
        -
        \cF^{(I)}_q
    \Vert
    }
    {
    \tau
    +
    \Vert
        \cF^{(I)}_p
        -
        \cF^{(I)}_q
    \Vert
    }~,
\end{align}
where $\tau>0$ is a threshold distance between embeddings. We prune all edges $(p,q)$ for which $d(p,q)<0.5$, \ie $\Vert\cF^{(I)}_p - \cF^{(I)}_q\Vert> \tau$.
We then define superpoints as the connected components of the resulting graph.

We set a minimal size $\sizemin$ for superpoints. Superpoints containing fewer than $\sizemin$ points are merged with the neighbouring superpoints (\ie, superpoints containing each end of a neighbourhood $(p,q)$ with $q \in \cN(p)$ or $q \in \cN(p)$)
as induced by the point adjacency relationship $\cN$.

\para{Hierarchal Partitioning?} 

\para{Training.}
\begin{align}
    \cL = 
    \sum_{p,q \in E^{\text{inter}}}\focal(d(p,q))
    +
    \sum_{p,q \in E^{\text{intra}}}\focal(1-d(p,q))~,
\end{align}
where $\focal(y)=-(1-y)^\gamma \log(y)$ with $\gamma>0$ an hyper-parameter.

\subsection{}

\subsection{Implementration Details}


\subsection{Greedy Low Contour Prediction}
The partition provided by Mean Shift tend to be over-segmented with staircaising effects. We can improve this by adding a low-contour prior. We propose an heuristic to solve this purely in GPU.

We denote $x$ the features provided by MS. Wse denote by $\cP$ the partiton.

We denote: 
\begin{align}
x_P = \frac1{\Vert P \Vert}\sum_{p \in P} x_p
\end{align}

We want to minimize an energy:
\begin{align}
H(\cP)
&=
\sum_{P \in \cP} 
    \sum_{p \in P} 
    \Vert x_p - x_P \Vert^2
+
\regul
\sum_{(p,q)\in E}
    w_{p,q}
    \Vert x_p - x_q \Vert_0 \\
&=
% \sum_{P \in \cP} \Vert P \Vert
% \sum_{p \in P} \Vert x_p  %\Vert^2
% - 
% \Vert x_P \Vert^2 \\
\sum_{P \in \cP} \left( 
\sum_{p \in P} \Vert x_p   \Vert^2
- \Vert P \Vert \Vert x_P \Vert^2 
\right) 
+
\regul
\sum_{(P,Q)\in E}
    w_{P,Q}  
\end{align}

We now consider the partition $\cP'$ where $P$ and $Q$ are merged into one single superpoint $R$

\begin{align}\nonumber
H(\cP')
&=
% \sum_{P \in \cP'} \Vert P \Vert
% \sum_{p \in P} \Vert x_p  \Vert^2
% - 
% \Vert x_P \Vert^2 
\sum_{P \in \cP'} \left( 
\sum_{p \in P} \Vert x_p
- \Vert P \Vert \Vert x_P \Vert^2 
\Vert^2
\right) 
+\\
&\regul
\left( 
\sum_{(U,V)\in E}
    w_{U,V} 
- w_{P,Q}
\right) 
\end{align}



We consider by merging $P$ and $Q$ into a new SP $R$.
\begin{align}\nonumber
    x_R 
    &= \frac1{\Vert P  \Vert + \Vert Q \Vert}
    \sum_{p \in P \cup Q} x_p \\
    &=\frac
    {\Vert P \Vert x_P + \Vert Q \Vert x_Q}
    {\Vert P  \Vert + \Vert Q \Vert}
\end{align}


We compute $\Delta(P,Q)$ the gain in energy of this merge:
\begin{align}\nonumber
    \Delta(P,Q) 
    &= H(\cP') - H(\cP)\\\nonumber
    &=  
   -\Vert R \Vert \Vert x_R \Vert^2 + 
    \sum_{p \in P \cup Q} \Vert x_p  \Vert^2 \\\nonumber
    &+  \Vert P \Vert  \Vert x_P \Vert^2 +  \Vert Q \Vert  \Vert x_Q \Vert^2
    - \sum_{p \in P \cup Q} \Vert x_p  \Vert^2 \\\nonumber
    & - \regul w_{P,Q} \\
    & = \Vert P \Vert \Vert x_P \Vert^2 + \Vert Q \Vert \Vert x_Q \Vert^2 - \Vert R \Vert \Vert x_R \Vert^2 - \regul w_{P,Q} \\
    & = \frac{\Vert P \Vert \Vert Q \Vert}{\Vert P \Vert + \Vert Q \Vert} \Vert x_P - x_Q \Vert^2 - \regul w_{P,Q}
\end{align}


==> tables/results.tex <==
\centering\small{{
    \setlength{\tabcolsep}{4pt} 
    \begin{tabular}{l c c cc c c}\toprule
        \multirow{2}{*}{Model} 
        &
        Throughput
        &
        Size
        &
        \multicolumn{2}{c}{S3DIS}
        &
        \multicolumn{1}{c}{KITTI}
        &
        \multirow{2}{*}{DALES}
        \\\cmidrule(lr){4-5}
        & Kpt/s
        & $\times10^6$
        & \footnotesize{6-Fold}  & \footnotesize{Area~5} & \multicolumn{1}{c}{360 val} &%\multicolumn{1}{c}
        \\ \midrule 
        PointNet++ \cite{qi2017pointnetpp}& 1400 & \hphantom{4}3.0 & 56.7   & - & - & 68.3  \\
        %PointNeXt-S \cite{qian2022pointnext}& 0.8 & 68.0 & 64.2 & - & - \\
        %ConvPoint \cite{boulch2020convpoint} & ?  &\hphantom{4}4.7& 68.2 & - & - & 67.4 \\
        %$\dagger$ {SPG + SSP \cite{landrieu2019point}}& ? &  0.29 & 68.4 & 61.7 & - & -  \\
        %$\dagger$ SPNet \cite{hui2021superpoint} & ? & 0.32 & 68.7 &-&-&- \\
        MinkowskiNet \cite{choy20194d,chaton2020torch}& 430 & 37.9& 69.1 & 65.4& 58.3 & - \\
        %RandLANet \cite{hu2020randla}& ? & \hphantom{4}1.2 &  70.0&- & - & - \\
        KPConv \cite{thomas2019kpconv}& 274 & 14.1& 70.6 & 67.1 & - & \bf 81.1 \\
        %PTv2\cite{zhao2021point}& ? & \hphantom{4}7.8 & 73.5 & 70.4  & - & - \\
        %RepSurf-U \cite{ran2022surface}& ?& 0.97 &74.3 & 68.9 & - & - \\
        %DeepViewAgg \cite{robert2022learning}& ? & 41.2 & 74.7 & 67.2  & 62.1 & -\\ 
        Stratified Trans. \cite{lai2022stratified,Wang2022WindowNE} & ? & \hphantom{0}8.0 & 74.9 & 72.0 & - & 74.3 \\ 
        PointNeXt-XL \cite{qian2022pointnext}& 4.1 & 41.6 & 74.9 & 71.1  & - & - \\
        %Swin3D & ? & 60.8 & 76.9 & 72.5 \\
        PTv3 \cite{wu2024point} & 24.7 & 46.2 & \bf  77.7 & \bf  73.4 & & \\
        \greyrule
        $\dagger$ SPG \cite{landrieu2018spg} & 134 &0.28 & 62.1 & 58.0 & - & 60.6  \\
        $\dagger$ SPNet \cite{hui2021superpoint} & ? & 0.33 & 68.7 & - & - & -  \\
        $\dagger$ SPT \cite{robert2023efficient} & 1168 &  0.21 & 76.0 & 68.9 & \bf 63.5 & 79.6 \\
        \midrule
        $\dagger$ \bf Easy-SP + SPT (ours) & 2500 \\
        \midrule
        \bottomrule
    \end{tabular}
}}

==> tables/speed.tex <==


    \small 
    \begin{tabular}{l cccc c}
    \toprule
    & pre-processing & partition & inference & total & training \\ 
    \cmidrule(lr){2-5} \cmidrule(lr){6-6}
    & \multicolumn{4}{c}{all 6 areas of S3DIS, in \unit{\second}} & one fold, in GPU-h \\
    \midrule
    PointNet++ \cite{qi2017pointnetpp}                          &  125 & - & 133 &  258 & 1.6 \\
    KPConv \cite{thomas2019kpconv}                              & 1031 & - & 900 & 1931 & 18.8 \\
    MinkowskiNet \cite{choy20194d}                              &  887 & - & 767 & 1654 & \TODO{28.8} \\
    PointNeXt-XL \cite{qian2022pointnext}                       &    - & - & 168426 & 168426 & 82.9 \\
    Stratified Trans. \cite{lai2022stratified,Wang2022WindowNE} &    - & - &  67216 & 67216 & 216.4 \\
    PTv3 \cite{wu2024point}                                     &    - & - & 28206 & 28206 & 88 \\ \greyrule
    SPG \cite{landrieu2018spg}                                  & 3187 & 2616 & 142 & 5945 & \TODO{1.3} \\
    SSP \cite{landrieu2018spg}                                  & 3270 & 2616 & 142 & 6028 & \TODO{1.3 + ?} \\    
    SPNet \cite{hui2021superpoint}                              & 3187 & 1132 & 142 & 4461 & \TODO{7 ?} \\
    SPT \cite{robert2023efficient}                              &  306 & 271 & \TODO{18 ?} & \TODO{596} & \TODO{3.0} \\
    \greyrule
    \bf EasySP (ours)                                           &  \TODO{305} & \TODO{1} & \TODO{18} & \TODO{325} \\
    \bottomrule
    \end{tabular}



==> templates/3DV/preamble.tex <==
%
% --- inline annotations
%
\usepackage[dvipsnames]{xcolor}
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
% --- disable by uncommenting  
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}


